Unsupervised Intuitive Physics from Past Experiences

We are interested in learning models of intuitive physics similar to the ones that animals use for navigation, manipulation and planning. In addition to learning general physical principles, however, we are also interested in learning ``on the fly'', from a few experiences, physical properties specific to new environments. We do all this in an unsupervised manner, using a meta-learning formulation where the goal is to predict videos containing demonstrations of physical phenomena, such as objects moving and colliding with a complex background. We introduce the idea of summarizing past experiences in a very compact manner, in our case using dynamic images, and show that this can be used to solve the problem well and efficiently. Empirically, we show via extensive experiments and ablation studies, that our model learns to perform physical predictions that generalize well in time and space, as well as to a variable number of interacting physical objects.

==> fig-dataset.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=.24\linewidth]{./images/pic_0001}
\includegraphics[width=.24\linewidth]{./images/pic_0003}
\includegraphics[width=.24\linewidth]{./images/pic_0005}
\includegraphics[width=.24\linewidth]{./images/pic_003}
\caption{Dataset sample images}
\label{fig:sample}
\end{figure}

==> tab-multiple_balls.tex <==
%\begin{table*}[t]
%  \centering
%  \caption{\textbf{Tempral invariance on Normal-3 balls unsupervised}, Number of balls over time}\label{t:normal-1ball-uns}
%  %\vspace{-1em}
%  \scriptsize
%  \setlength{\tabcolsep}{0.4em}
%
%  \sisetup{detect-weight=true,detect-inline-weight=math,  table-column-width=4.2em}
%  \newcommand{\boldentryy}[2]{%
%  \multicolumn{1}{S[table-format=0.3,
%                      mode=text, text-rm=\fontseries{b}\selectfont
%                     ]#2}{#1}}
%  \newcolumntype{F}{S[table-format=0.3,table-column-width=4.2em]}
%  \begin{tabular}{ccccc}
%  \toprule
%      & \multicolumn{4}{c}{Normal-3 ball-\Ttrain=20}\\
%      Method &
%     \multicolumn{1}{c}{$T=$6} & \multicolumn{1}{c}{$T=$\Ttrain} &    \multicolumn{1}{c}{$3\times$\Ttrain} & 
%      \multicolumn{1}{c}{$5\times$\Ttrain}\\ 
%      64x64 + 1 ball trained + Perc. loss & 3.1 $\pm$0.5 & 2.8$\pm$0.9 & 1.7$\pm$0.8 & 1.5$\pm$0.8\\
%  %    \midrule
%  \end{tabular}
%  \end{table*}
  
  
  
\begin{table*}[t]
\centering
\footnotesize
\newcommand{\xpm}[1]{{\tiny$\pm$#1}}
\caption{\textbf{Predicting multiple moving object.} Obstacle type is R2, all network were trained on the fully unsupervised with perceptual loss. Num. is the maxmium number of balls per run during training. For instance Num=3 means that every runs sampled contained one to three balls.
The test board is size $64\times 64$
We test the average prediction error at $T_{\text{test}}=20,60,100$ well above the duration $T_\text{train}=20$ observed during training.
}
\label{t:normal-mul-uns}
\setlength{\tabcolsep}{0.21em}
\begin{tabular}{c*2c*2c*2c}
\toprule
& \multicolumn{2}{c}{$T_\text{test} = T_{\text{train}} = 20$} & \multicolumn{2}{c}{$T_\text{test} = 3\times$\Ttrain} &  \multicolumn{2}{c}{$T_\text{test}=5\times$\Ttrain}\\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\\
Num.  & \# obj.     & Vid.~$L_2$    & \# obj.      & Vid.~$L_2$      &  \# obj.      & Vid.~$L_2$      \\
\midrule
\multicolumn{7}{c}{3 Balls}\\
\midrule
1  & 2.6\xpm{0.8} & 6.5\xpm{5.2}  &  1.7\xpm{0.9}  & 8.5\xpm{5.9}    & 1.6\xpm{0.8}  & 8.5\xpm{6.0}  \\
3 &  3.1\xpm{0.6} & 4.6\xpm{4.8} & 2.9\xpm{0.8}  & 10.4\xpm{7.6}   & 2.9\xpm{0.9}  & 11.0\xpm{8.0} \\
\midrule
\multicolumn{7}{c}{5 Balls}\\\midrule

1  & 3.3\xpm{1.0} & 8.9\xpm{6.6}   & 2.0\xpm{1.0}  & 10.2\xpm{7.4}   &  3.1\xpm{0.6}  & 1.8\xpm{.775}  \\
3 &  5.5\xpm{0.7} & 6.6\xpm{6.2} & 5.1\xpm{1.1}  & 13.0\xpm{9.5}   &  5.1\xpm{1.0}  & 13.5\xpm{10.0} \\
%\multicolumn{7}{c}{3 Balls}\\
%\midrule
%1  & 2.6\xpm{0.8} & .46\xpm{.30}  & 1.7\xpm{0.9}  & .8\xpm{.39}   & 1.6\xpm{0.8}  & .79\xpm{.40} \\
%3 &  3.1\xpm{0.6} & .23\xpm{.26}& 2.9\xpm{0.8}  & 1.20\xpm{.63}  & 2.9\xpm{0.9}  & 1.35\xpm{.71} \\
%\midrule
%\multicolumn{7}{c}{5 Balls}\\
%\midrule
%
%1  & 3.3\xpm{1.0} & .88\xpm{.48}   & 2.0\xpm{1.0}  & 1.15\xpm{.61} & 3.1\xpm{0.6}  & 1.17\xpm{.65} \\
%3 &  5.5\xpm{0.7} & .49\xpm{.42} & 5.1\xpm{1.1}  & 1.85\xpm{.99}   &  5.1\xpm{1.0}  & 2.03\xpm{1.11} \\
\bottomrule
\end{tabular}
\end{table*}

\if0 %BEFORE RENORM
\begin{table*}[t]
\centering
\footnotesize
\newcommand{\xpm}[1]{{\tiny$\pm$#1}}
\caption{\textbf{Predicting multiple moving object.} Obstacle type is R2, all network were trained on the fully unsupervised with perceptual loss. Num. is the maxmium number of balls per run during training. For instance Num=3 means that every runs sampled contained one to three balls.
The test board is size $64\times 64$
We test the average prediction error at $T_{\text{test}}=20,60,100$ well above the duration $T_\text{train}=20$ observed during training.
Video prediction error has been normalized by the board size diagonal.
}
\label{t:normal-mul-uns}
\setlength{\tabcolsep}{0.21em}
\begin{tabular}{c*2c*2c*2c}
\toprule
& \multicolumn{2}{c}{$T_\text{test} = T_{\text{train}} = 20$} & \multicolumn{2}{c}{$T_\text{test} = 3\times$\Ttrain} &  \multicolumn{2}{c}{$T_\text{test}=5\times$\Ttrain}\\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}\\
Num.  & \# obj.     & Vid.~$L^2$    & \# obj.      & Vid.~$L^2$      &  \# obj.      & Vid.~$L^2$      \\
\midrule
\multicolumn{7}{c}{3 Balls}\\
1  & 2.6\xpm{0.8} & 42.11\xpm{27.2}  &  1.7\xpm{0.9}  & 72.4\xpm{35.4}    & 1.6\xpm{0.8}  & 72.0\xpm{36.6}  \\
3 &  3.1\xpm{0.6} & 21.2\xpm{23.3} & 2.9\xpm{0.8}  & 108.4\xpm{57.4}   & 2.9\xpm{0.9}  & 122.0\xpm{63.8} \\
\midrule
\multicolumn{7}{c}{5 Balls}\\\midrule

1  & 3.3\xpm{1.0} & 79.5\xpm{43.8}   & 2.0\xpm{1.0}  & 104.7\xpm{55.3}   &  3.1\xpm{0.6}  & 3.1\xpm{0.6}  \\
3 &  5.5\xpm{0.7} & 44.2\xpm{38.2} & 5.1\xpm{1.1}  & 168.2\xpm{90.0}   &  5.1\xpm{1.0}  & 183.6\xpm{100.8} \\
%\multicolumn{7}{c}{3 Balls}\\
%\midrule
%1  & 2.6\xpm{0.8} & .46\xpm{.30}  & 1.7\xpm{0.9}  & .8\xpm{.39}   & 1.6\xpm{0.8}  & .79\xpm{.40} \\
%3 &  3.1\xpm{0.6} & .23\xpm{.26}& 2.9\xpm{0.8}  & 1.20\xpm{.63}  & 2.9\xpm{0.9}  & 1.35\xpm{.71} \\
%\midrule
%\multicolumn{7}{c}{5 Balls}\\
%\midrule
%
%1  & 3.3\xpm{1.0} & .88\xpm{.48}   & 2.0\xpm{1.0}  & 1.15\xpm{.61} & 3.1\xpm{0.6}  & 1.17\xpm{.65} \\
%3 &  5.5\xpm{0.7} & .49\xpm{.42} & 5.1\xpm{1.1}  & 1.85\xpm{.99}   &  5.1\xpm{1.0}  & 2.03\xpm{1.11} \\
\bottomrule
\end{tabular}
\end{table*}
\fi

==> tab-num-runs-sup.tex <==
\begin{table*}[t]
\centering
\scriptsize
\newcommand{\xpm}[1]{{\tiny$\pm$#1}}
\setlength{\tabcolsep}{0.5em}
\caption{\textbf{Importance of experience.} For the \textbf{supervised} model, we report the trajectory prediction error at $T=40$ (rows 1-3) and the obstacle map prediction error (rows 4-6) for different obstacle types.
The number of runs $N$ in the experiences is varied from 0 to 50.
%Values have been normalized by the board size diagonal.
Position errors were normalized by the board size diagonal. $T_\text{train} = 20$.
}\label{t:num_runs_pos}
\begin{tabular}{cllcccccccc}
\toprule
No  & Err. &  Obst.    & $N            = 0$            & $1$           & $2$           & $5$           & $7$           & $10$          & $20$ & $50$\\ 
\midrule
(1) & Pos. & R2   & 1.81\xpm{1.41} & .94\xpm{.975} & .53\xpm{.81} & .15\xpm{0.41}  & .08\xpm{.21}   & .07\xpm{.16}  & .10\xpm{.24}   & .19\xpm{.38} \\
(2) & Pos. & R4 & 3.28\xpm{1.94}  & 2.22\xpm{1.67} & 1.56\xpm{1.40} & .63\xpm{.84} & .43\xpm{.68} &  .37\xpm{.60} & .44\xpm{.61} & .83\xpm{.97}\\
(3) & Pos. &  C      & 1.05\xpm{0.91} & .58\xpm{.61} & .36\xpm{.49} & .15\xpm{.29} & .13\xpm{.26} & .12\xpm{.22} &  .16\xpm{.26} & .24\xpm{.36}\\
\midrule
(4) & Obs. &  R2   & 4.1\xpm{4.0} & 3.6\xpm{3.8} & 3.1\xpm{3.4 }& 2.3\xpm{2.5}  & 2.3\xpm{2.4}  & 2.3\xpm{2.4}  & 2.3\xpm{2.7}   & 2.6\xpm{3.0} \\
(5) & Obs. & R4 & 6.1\xpm{2.2}  & 4.1\xpm{3.8} & 3.1\xpm{3.4} & 2.8\xpm{3.3} & 2.7\xpm{3.1} & 2.6\xpm{3.0} & 2.7\xpm{2.9} & 3.3\xpm{3.6}\\
(6) & Obs. & C      & 3.9\xpm{3.9}  & 3.3\xpm{3.7} & 2.8\xpm{3.1} & 2.4\xpm{2.7} & 2.4\xpm{2.8} & 2.3\xpm{2.6} & 2.4\xpm{2.6} & 2.5\xpm{2.9}\\

%(4) & Obs. &  R2   & .178\xpm{.175} & .142\xpm{.160} & .107\xpm{.126 }& .060\xpm{.072}  & .056\xpm{.064}  & .056\xpm{.063}  & .061\xpm{.082}   & .075\xpm{.100} \\
%(5) & Obs. & R4 & .409\xpm{.053}  & .190\xpm{.158} & .107\xpm{.126} & .087\xpm{.118} & .801\xpm{.103} & .078\xpm{.103} & .081\xpm{.096} & .120\xpm{.140}\\
%(6) & Obs. & C      & .166\xpm{.171}  & .122\xpm{.152} & .084\xpm{.108} & .061\xpm{.078} & .640\xpm{.088} & .061\xpm{.072} & .061\xpm{.074} & .072\xpm{.096}\\
\bottomrule
\end{tabular}
\end{table*}

\if0
\begin{table*}[t]
\centering
\scriptsize
\newcommand{\xpm}[1]{{\tiny$\pm$#1}}
\setlength{\tabcolsep}{0.5em}
\caption{\textbf{Importance of experience.} For the \textbf{supervised} model, we report the trajectory prediction error at $T=40$ (rows 1-3) and the obstacle map prediction error (rows 4-6) for different obstacle types.
The number of runs $N$ in the experiences is varied from 0 to 50.
Values have been normalized by the board size diagonal.
}\label{t:num_runs_pos}
\begin{tabular}{cllcccccccc}
\toprule
No  & Err. &  Obst.    & $N            = 0$            & $1$           & $2$           & $5$           & $7$           & $10$          & $20$ & $50$\\ 
\midrule
(1) & Pos. & R2   & 1.81\xpm{1.41} & .94\xpm{.975} & .53\xpm{.81} & .15\xpm{0.41}  & .08\xpm{.21}   & .07\xpm{.16}  & .10\xpm{.24}   & .19\xpm{.38} \\
(2) & Pos. & R4 & 3.28\xpm{1.94}  & 2.22\xpm{1.67} & 1.56\xpm{1.40} & .63\xpm{.84} & .43\xpm{.68} &  .37\xpm{.60} & .44\xpm{.61} & .83\xpm{.97}\\
(3) & Pos. &  C      & 1.05\xpm{0.91} & .58\xpm{.61} & .36\xpm{.49} & .15\xpm{.29} & .13\xpm{.26} & .12\xpm{.22} &  .16\xpm{.26} & .24\xpm{.36}\\
\midrule
(4) & Obs. &  R2   & 16.9\xpm{15.9} & 12.9\xpm{14.5} & 9.7\xpm{11.4 }& 5.4\xpm{6.5}  & 5.1\xpm{5.8}  & 5.1\xpm{5.8}  & 5.5\xpm{7.4}   & 6.8\xpm{9.1} \\
(5) & Obs. & R4 & 37.0\xpm{4.8}  & 17.2\xpm{14.3} & 9.7\xpm{11.4} & 7.9\xpm{10.7} & 7.1\xpm{9.4} & 7.0\xpm{9.3} & 7.4\xpm{8.7} & 10.9\xpm{12.7}\\
(6) & Obs. & C      & 15.0\xpm{15.5}  & 11.1\xpm{13.8} & 7.6\xpm{9.8} & 5.6\xpm{7.1} & 5.8\xpm{8.0} & 5.5\xpm{6.6} & 5.6\xpm{6.7} & 6.5\xpm{8.7}\\

%(4) & Obs. &  R2   & .178\xpm{.175} & .142\xpm{.160} & .107\xpm{.126 }& .060\xpm{.072}  & .056\xpm{.064}  & .056\xpm{.063}  & .061\xpm{.082}   & .075\xpm{.100} \\
%(5) & Obs. & R4 & .409\xpm{.053}  & .190\xpm{.158} & .107\xpm{.126} & .087\xpm{.118} & .801\xpm{.103} & .078\xpm{.103} & .081\xpm{.096} & .120\xpm{.140}\\
%(6) & Obs. & C      & .166\xpm{.171}  & .122\xpm{.152} & .084\xpm{.108} & .061\xpm{.078} & .640\xpm{.088} & .061\xpm{.072} & .061\xpm{.074} & .072\xpm{.096}\\
\bottomrule
\end{tabular}
\end{table*}
\fi

==> tab-num-runs.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{\textbf{Effect of experience on learning about the obstacles.} We report the $L^2$  ... ? \todo{How do you do this with the unsupervised model? We should probably report the impact on trajectory prediction instead.} $L_2$ loss between background prediction from network and ground truth.
In all experiments we compare predicted obstacle map from supervised model and the ground truth.
For each data generation procedure we vary the number of runs $N$ used to predict the background.
Additionally we show the predictions error when we assume every object is an obstacle.\todo{Maybe do it on the unsupervised model? AV: yes}}\label{t:num_runs}
\begin{tabular}{cccccccccc}
\toprule
Data           & $N=0$ (all obst.)            & $N=0$               & $1$             & $2$             & $5$             & $7$             & $10$            & $20$            & $50$\\ 
\midrule
Normal         & 173.8$\pm$123.8 & 126.6$\pm$164.5 & 90.6$\pm$85.5 & 77.4$\pm$52.1 & 10.6$\pm$29.6 & 7.8$\pm$22.1  & 7.8$\pm$21.8  & 12.6$\pm$32.9 & 21.4$\pm$41.6 \\
n-[[3,4] obst. & 283.5$\pm$177.9 &\\
Custom         & 88.4$\pm$78.5   & 96.2$\pm$82.3   & 55.2$\pm$57.0 & 36.4$\pm$48.5 & 15.6$\pm$27.5 & 14.4$\pm$27.2 & 12.1$\pm$23.0 & 14.3$\pm$25.2 & 20.5$\pm$32.1\\
\bottomrule
\end{tabular}
\end{table*}

%\begin{tabular}{cccccccccc}
%\toprule
%Data           & Ref.            & $N=0$               & $1$             & $2$             & $5$             & $7$             & $10$            & $20$            & $50$\\ 
%\midrule
%Normal         & 173.0$\pm$123.3 & 126.6$\pm$164.5 & 90.6$\pm$85.5 & 77.4$\pm$52.1 & 10.6$\pm$29.6 & 7.8$\pm$22.1  & 7.8$\pm$21.8  & 12.6$\pm$32.9 & 21.4$\pm$41.6 \\
%n-[[3,6] obst.\\
%Custom         & 87.8$\pm$78.4   & 96.2$\pm$82.3   & 55.2$\pm$57.0 & 36.4$\pm$48.5 & 15.6$\pm$27.5 & 14.4$\pm$27.2 & 12.1$\pm$23.0 & 14.3$\pm$25.2 & 20.5$\pm$32.1\\
%Custom+Texture & 87.8$\pm$78.4   & 97.0$\pm$83.0   & 55.4$\pm$62.7 & 32.2$\pm$49.0 & 10.6$\pm$26.4 & 8.7$\pm$22.2  & 6.7$\pm$12.1  & 7.5$\pm$11.2  & 11.2$\pm$16.5\\
%\bottomrule
%\end{tabular}
%\end{table*}


==> tab-temporal-inv-custom.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{Tempral invariance on Custom 1-ball.}}\label{t:normal-1ball}
  %\vspace{-1em}
  \scriptsize
  \sisetup{detect-weight=true,detect-inline-weight=math,  table-column-width=4.0em}
  \newcommand{\boldentryy}[2]{%
  \multicolumn{1}{S[table-format=0.1,
                      mode=text, text-rm=\fontseries{b}\selectfont
                     ]#2}{#1}}
  \newcolumntype{F}{S[table-format=0.1,table-column-width=4.0em]}
  \begin{tabular}{c*3F*3F*3F}
  \toprule
      & \multicolumn{9}{c}{Normal-1 ball-\Ttrain=20}\\
      \cmidrule(lr){2-10}
      Method &
     \multicolumn{3}{c}{$T=$\Ttrain} &    \multicolumn{3}{c}{$3\times$\Ttrain} & 
      \multicolumn{3}{c}{$5\times$\Ttrain}\\ 
      \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}\\
      & \multicolumn{1}{c}{N}  & \multicolumn{1}{c}{Im}  & \multicolumn{1}{c}{Pos} &  \multicolumn{1}{c}{N}  & \multicolumn{1}{c}{Im}  & \multicolumn{1}{c}{Pos} &\multicolumn{1}{c}{N}  & \multicolumn{1}{c}{Im}  & \multicolumn{1}{c}{Pos} \\
      \midrule
      Bgd $L_2$ &  1.0$\pm$0.2 & 5.3$\pm$9.4 & 1.9$\pm$5.8 &  0.1$\pm$0.3& 19.4$\pm$14.6 & 43.7$\pm$19.3 & 0.0$\pm$0.1 & 20.3$\pm$13.6& 48.4$\pm$17.6\\
      Bgd $L_2$ + Perc.
      loss & 1.0$\pm$0.0 & 6.7$\pm$10.7 & 1.6$\pm$2.2 & 1.0$\pm$0.1 & 29.2$\pm$21.9 & 12.4$\pm$10.2 & 1.0$\pm$0.2 & 29.3$\pm$20.4 &21.7$\pm$12.3\\
      No Bgd  $L_2$ & 1.0$\pm$0.2 & 9.9$\pm$6.6 & 4.3$\pm$10.7 & 0.3$\pm$0.5 & 18.1$\pm$13.3 & 39.9$\pm$20.2 & 0.2$\pm$0.5 & 19.1$\pm$13.8 &44.9$\pm$18.7\\
      No Bgd $L_2$ + Perc.
      loss & 1.0$\pm$0.5 & 7.1$\pm$10.7 & 3.2$\pm$7.9 & 0.9$\pm$0.4 & 24.0$\pm$18.0 & 20.2$\pm$16.8 & 0.9$\pm$0.5 & 24.4$\pm$17.3 &28.6$\pm$16.2\\
  %    \midrule
  \end{tabular}
  \end{table*}
  

==> tab-temporal-inv.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Temporal invariance on Normal-1 ball.} Trained with perceptual loss}\label{t:normal-1ball}
%\vspace{-1em}
\scriptsize
\sisetup{detect-weight=true,detect-inline-weight=math,  table-column-width=4.0em}
\newcommand{\boldentryy}[2]{%
\multicolumn{1}{S[table-format=0.1,
                mode=text, text-rm=\fontseries{b}\selectfont
                ]#2}{#1}}
\newcolumntype{F}{S[table-format=0.1,table-column-width=4.0em]}
\begin{tabular}{c*3c*3c*3c}
\toprule
& \multicolumn{9}{c}{Normal-1 ball-\Ttrain=20}\\
\cmidrule(lr){2-10}
Method &
\multicolumn{3}{c}{$T=$\Ttrain} &    \multicolumn{3}{c}{$3\times$\Ttrain} & 
\multicolumn{3}{c}{$5\times$\Ttrain}\\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}\\
& \multicolumn{1}{c}{N}  & \multicolumn{1}{c}{Im}  & \multicolumn{1}{c}{Pos} &  \multicolumn{1}{c}{N}  & \multicolumn{1}{c}{Im}  & \multicolumn{1}{c}{Pos} &\multicolumn{1}{c}{N}  & \multicolumn{1}{c}{Im}  & \multicolumn{1}{c}{Pos} \\
\midrule
64x64 & 1.0$\pm$0.1 & 9.1$\pm$11.8 & 1.6$\pm$2.3 & 1.0$\pm$0.2 & 32.5$\pm$18.8 & 9.6$\pm$7.3 & 1.0$\pm$0.3 & 33.4$\pm$17.6 &19.6$\pm$11.8\\
128x128 & 8.3$\pm$3.3 & 94.5$\pm$57.2 & 8.65$\pm$6.8 & 26.8$\pm$6.9 & 504.3$\pm$259.0 & 17.9$\pm$10.5 & 26.3$\pm$7.6 & 540.4$\pm$279.7 &20.8$\pm$11.7\\
%    \midrule
\end{tabular}
\end{table*}

